Calculating and Visualizing Counterfactual Feature Importance Values

Despite the success of complex machine learning algorithms, mostly justified by an outstanding performance in prediction tasks, their inherent opaque nature still represents a challenge to their responsible application. Counterfactual explanations surged as one potential solution to explain individual decision results. However, two major drawbacks directly impact their usability: (1) the isonomic view of feature changes, in which it is not possible to observe \textit{how much} each modified feature influences the prediction, and (2) the lack of graphical resources to visualize the counterfactual explanation. We introduce Counterfactual Feature (change) Importance (CFI) values as a solution: a way of assigning an importance value to each feature change in a given counterfactual explanation. To calculate these values, we propose two potential CFI methods. One is simple, fast, and has a greedy nature. The other, coined CounterShapley, provides a way to calculate Shapley values between the factual-counterfactual pair. Using these importance values, we additionally introduce three chart types to visualize the counterfactual explanations: (a) the Greedy chart, which shows a greedy sequential path for prediction score increase up to predicted class change, (b) the CounterShapley chart, depicting its respective score in a simple and one-dimensional chart, and finally (c) the Constellation chart, which shows all possible combinations of feature changes, and their impact on the model's prediction score. For each of our proposed CFI methods and visualization schemes, we show how they can provide more information on counterfactual explanations. Finally, an open-source implementation is offered, compatible with any counterfactual explanation generator algorithm. Code repository at: https://github.com/ADMAntwerp/CounterPlots

==> alg1_old.tex <==
% algorithm to calculate greedy scores

\begin{algorithm}[h]
\SetKwFunction{subsetlen}{getCoalitionsOfLength}
\caption{Calculating the greedy score vector ($\boldsymbol{\varrho}$) for a factual ($\textbf{x}$) and counterfactual ($\textbf{c}$) instances}
\label{alg:calcgreedy}
\KwIn{Prediction model ($\mathcal{M}$), factual ($\textbf{x}$) and counterfactual ($\textbf{x}$) points}
\KwOut{Vector with Greedy scores for each input feature 
($\boldsymbol{\varrho}$)}
$\boldsymbol{\varrho} \gets zeros(1,N)$\;
$\boldsymbol\delta \gets \textbf{c}-\textbf{x}$\;
$idx\_feats\_included \gets <>$\;
$mask_{\boldsymbol{\rho}} \gets eye(N)$\;
$\textbf{c}^* \gets \textbf{x}$\;
\For{$L \gets 0$ \KwTo $N$}{
    \tcp{Create a matrix with}
    \tcp{each feature modification}
    $\textbf{S}^* \gets \mathcal{M}(\textbf{c}^* + \boldsymbol{\delta} \cdot mask_{\boldsymbol{\varrho}} )$\;
    \tcp{Remove already modified features}
    $\textbf{S}^*.drop\_rows(idx\_feats\_included)$\;
    \tcp{Get the feature which most}
    \tcp{increased prediction score}
    $idx\_max\_change \gets arg\_max(\textbf{S}^*)$\;
    \tcp{Assign feature score}
    $\boldsymbol{\varrho}[idx\_max\_change] \gets max(\textbf{S}^*)$\;
    \tcp{Update counterfactual}
    $\textbf{c}^*[idx\_max\_change] \gets \textbf{c}[idx\_max\_change]$\;
    \tcp{Include feature index}
    \tcp{as already modified}
    $idx\_feats\_included.insert(idx\_max\_change)$\;
    
    
}
\KwRet{$\boldsymbol{\varrho}$}
\end{algorithm}

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
Artificial intelligence (AI) has become capable of capturing, learning and predicting complex data structures. The performance of GPT-3, for example, is good enough such that a piece of software can mimic language to a level that is often indistinguishable from human-written text. Deep learning models are capable of learning the intonation, tone and pronunciation habits of any voice with a sound excerpt of just a couple of seconds long as training data.
Learning highly complex data structures, such as speech, generally requires an equally complex model in order to accurately capture the nuances of the data. While this increase in complexity opens up the possibility of increased performance, it comes with a price: its explainability is greatly reduced. \todo{talk why explainability is important}. A model that is inexplicable due to its high number of parameters is called a "black box" model.
There exist many ways to invoke explainability in a black box model. These methods are often distinguished into two main categories: global or local.
Local explanation methods aim at uncovering why a model predicts some outcome for a singular data instance. Popular methods include, but are not limited to: assuming a locally linear decision boundary (i.e. LIME \todo{cite lime}), calculating the shapley values of the features of one instance (i.e. SHAP \todo{cite shap}), finding a similar instance with a different model outcome (i.e. counterfactual explanations) etc.
Global explanation methods aim at uncovering the inner workings of an entire model, independent of the input data. Such methods include, but are not limitid to: fitting a second explainable model to the initial inexplicable model (e.g. fitting a decision tree to a neural network such that it has similar performance), calculating an aggregated per-instance feature contribution (e.g. averaging all the shapley values of all instances) etc.
With the exception of counterfactual explanations, all listed explanation methods include ways to visualise the feature importances. Lime allows bar charts to visualise the weights of the locally linear decision boundary. SHAP allows many visual methods to compare the feature shapley values, such as waterfall plots, force plots, the popular beeswarm and violin plots, and even image plots for image recognition models.
By nature, the core idea of counterfactual explanations do not easily lend themselves to visualisation; it is next to impossible to visualise a data instance in multi-dimensional space. The output of a counterfactual explanation method, however, is a set of feature names and associated values that are to be changed. It is possible to visualise these, in much the same ways that SHAP visualisations work.
This work will showcase a number of ways to visualise counterfactual explanation methods.

==> motivation.tex <==
\section{motivation}
\label{sec:motivation}
Talk about why it is important to visualise these things:
- 

Talk about the conscious choice to make it look like SHAP, and the fact that it is quicker and better to do it with CF instead (lower dimensionality, often no need for approx-SHAP)

1. For users: instead of just having a set of features: its better to have a visualisation to get a better understanding.\\
2. To assess the quality of the cf itself\\
3. to spur new research (see the straight walk shapley plot)\\

\subsection{Research questions}
\begin{enumerate}
\item how to assign scores to features in cf explanation
\begin{enumerate}
    \item Exact shapley on cf: possible due to low amount of features
    \item Approx shapley (check paper from foster and david, julie moeyersoms)
    \item best first strategy (greedy)
\end{enumerate}

\item how to visualize this course
\begin{enumerate}
    \item force plot
    \item waterfall
    \item single line (TODO)
\end{enumerate}

\item How to assess the viz. What metric to use to assess if the viz is "good" $\xrightarrow[]{}$ preference study?
\end{enumerate}

\subsection{Future research}
\begin{enumerate}
    \item Feature correlation
    \item Show vicinity of cf: are all closeby points also cf?
\end{enumerate}



==> shapley_explanation.tex <==
\section{Shapley values explained for counterfactuals}
Consider an $N \times M$ dataset, with a set of features
\begin{equation}
    \textbf{F} = \{F_0, F_1, ... F_N\} 
\end{equation}

And instances
\begin{equation}
    \textbf{I}^m = \{I^m_0, I^m_1...I^m_N\}\ ,\ m \in \{0..M\}
\end{equation}

Each instance has specific values for $I^m_i, i \in \{0..N\}$. These values are used by a model $\mathcal{M}$ to assign a score $Q$. Scoring an instance with a model will be denoted by:
\begin{equation}
    \mathcal{M}(I^m) = Q
\end{equation}. 
If we consider a decision threshold $t$ of $\mathcal{M}$, assigning instances to class $A$ if $Q>t$ and to class $B$ if $Q<t$, we can effectively categorise all instances to either class.

One may now wonder, what exactly made it so that an instance was assigned to class $A$, rather than class $B$? Which feature values were important, and which weren't? What if we ever so slightly changed some feature value, would it have a big impact? Would the model assign a different class? How much could we change some feature values of an instance, such that the model would assign it to a different class?

Gaining insight in these questions is common practice of explainable AI, and can be categorised in
\begin{enumerate}
    \item Global explanations
    \item Local explanations
\end{enumerate}
\todo{explain counterfactuals in another section and ref back}
Finding counterfactual explanations are local explanations. A good counterfactual is commonly considered an instance (real or synthetic) that lies near the original instance, but has a different outcome class. What is considered to be ``near" can be measured on two metrics:
\begin{enumerate}
    \item As little feature changes as possible
    \item as small feature changes as possible
\end{enumerate}

Counterfactual generating algorithms typically try to optimise either of these metrics, or both these metrics.

If we define $S$ as a coalition of features (i.e. some subset of features), one can then define a shapley value $\varphi_i^m$ as:
\begin{equation}
\label{eq:shapley}
    \varphi_i^m(\mathcal{M}) = \sum_{\textbf{S}^m \subseteq \textbf{I}^m\setminus\{I^m_i\}}\frac{|\textbf{S}|!(N - |\textbf{S}| - 1)!}{N!}\left(\mathcal{M}(\textbf{S} \cup \{I^m_i\}) - \mathcal{M}(\textbf{S})\right)
\end{equation}
where N is the total number of features and the sum extends over all subsets $S$ of instance $\textbf{I}^m$ not containing feature $i$.
Reading from right to left, this equation can be understood by:
\begin{enumerate}
    \item Evaluating the model outcomes of some subset of features containing $I^m_i$, and again for the exact same subset, but not containing $I^m_i$.
    \item Considering the difference in these two model outcomes.
    \item Weighing this difference, depending on how often this particular coalition may occur.
    \item Considering all possible coalitions
\end{enumerate}
This weighted sum is nothing more but the average marginal contribution of $I^m_i$ to the model outcome.

This can easily be applied for the case of counterfactuals. Let us consider a set of features and associated values $I^\Delta$ that are to be changed in order to go from a factual $\textbf{F}$ to a counterfactual $\textbf{C}F$:
\begin{equation}
    \textbf{I}^\Delta = \{I^\Delta_0, I^\Delta_1 ... I^\Delta_L\} \ , \ L  \leq N
\end{equation}
such that
\begin{equation}
 \textbf{I}^\Delta = \textbf{CF} - \textbf{F} \cap \textbf{CF} = \textbf{CF} \setminus \textbf{F}
\end{equation}

If we want to know how much some feature change $I^\Delta_l$ contributed to the change in model prediction score, then we can change these features from the factual to the counterfactual value one by one, each time evaluating the difference in model outcome. Of course, the order in which these features are changed will have an influence on the difference in model outcome. Changing some feature value of an instance if two previous values have already been changed will yield a different outcome that changing the exact same feature if no previous changes have been made yet. For this reason, we must consider every possible order in which some feature can be changed.

If we consider the example of a counterfactual $CF$ to a Factual $F$, such that the counterfactual differs from the factual by $5$ feature values:
\begin{equation}
    CF \setminus F = \textbf{I}^\Delta, |\textbf{I}^\Delta|=5
\end{equation}
Let us consider the case where we replace each feature value of the counterfactual by its corresponding counterfactual value. Let us count the amount of times $I^\Delta_0$ was changed as third feature. This corresponds to considering all coalitions $\textbf{S}$ of size $2$ that do not contain $I^\Delta_0$. 

\begin{equation}
    [\times\ \times\ I^\Delta_0\ \times\ \times]
\end{equation}

All the possible combinations where $F^\Delta_0$ is changed as third can be counted by considering which features are left to be filled in on the places of the $\times$. 

One should now try out every single combination of two features that can be added on the first two places, as these will influence what exact contribution the third change (i.e. $I^\Delta_0$) will yield. This is equivalent to the summation sign in Equation~\ref{eq:shapley}, but limited to only coalitions of size $2$.
Note that it does not matter in which order these first two features will be filled in. Any coalition of feature changes will pop up 2 times. This corresponds to the weight of $|\textbf{S}|!$ in Equation~\ref{eq:shapley}.
Also note that it now does not matter anymore which features will be changed later on. These have no influence on the model output difference yielded by changing $F^\Delta_0$ as third feature.
Of course, we now only considered the case where $I^\Delta_0$ was changed as third.
To gain a complete understanding of the influence of $I^\Delta_0$, we must also consider the cases where it was changed first, second, fourth, and last. This is equivalent to considering coalitions of every possible size that do not contain $I^\Delta_0$, which is equivalent to the summation sign in Equation~\ref{eq:shapley}, but now not limited anymore to a fixed coalition size.
The only thing that remains is to weigh this with the total amount of different feature permutations by dividing by $N!$, yielding Equation~\ref{eq:shapley}.

\subsection{Superiority of counterfactuals for shapley values: computational cost}
We discussed how one must consider every possible subset of features (i.e. coalition) in order to asses the shapley value of some feature. The amount of possible subsets for $N$ features is equal to \begin{equation}
    N_{coalitions} = \sum_{i}^N {N\choose i} = 2^N-1
\end{equation}
It is clear how this scales exponentially. When one considers only the shapley values for counterfactuals, the amount of possible subsets is
\begin{equation}
    N_{coalitions,CF} = \sum_{i}^L {L\choose i} = 2^L-1\ , \ L \leq N
\end{equation}

When a counterfactual algorithm is now optimised to minimise the amount of features that are to be changed in order to create a counterfactual, this can vastly reduce the amount of coalitions that are to be considered, and consequently, vastly reduce the computational cost of calculating shapley values. Of course, you only end up with shapely values of the features whose values differ between the factual and counterfactual.

\subsection{Superiority of counterfactuals for shapley values: improved insight}
The authors argue that, by limiting the calculation of shapley values to only include features associated with a counterfactual, not only does the computational cost reduce, but the explainability of a model improves as well. Comparing an instance to the average instance is rarely useful, and often we are not interested in the average prediction. For instance-based explanations, we are interested in answering the question ``Why did the model assign this particular class to this particular instance, \textbf{and how can I change it}?" While SHAP compares the instance to the average prediction score, this method compares the instance to a counterfactual, whose defining characteristic is exactly what is of importance here: a class switch. Not only does the counterfactual generator provide you with one or more coutnerfactual data points, already yielding a level of understanding in the model, the associated shapley values can also tell you how each of these feature changes contributed to the eventual class switch. The computational cost has effectively been outsourced to the counterfactual generating algorithm, thus separating the computational cost from the visualisation.

==> todo.tex <==

\section{Todo}
\begin{itemize}
\item explain shapley, explain why it is faster when first using counterfactuals (order of shaply and approx shapley), use formal definitions (see wikipedia)
    \item peer-reviewed conference with proceedings or journal
\item Viz should look nice
\item mailing list of people who work in counterfactuals, to check how they would like to use this library, and what they’re using
\item arxiv version, send it to people to test, get them to use it, only after that make pip version
\item maybe include UGent prof who gives data visualisaion course and was known for covid visualisations on VRT: \href{https://biblio.ugent.be/person/802000382679}{Bart Mesuere} (why was this a good idea again?)
\end{itemize}

\section{literature to check out}

\href{https://reader.elsevier.com/reader/sd/pii/S0167923610002368?token=4A8E742FCB3D54ED6C0D31FA4C097F93C3235C16689C055C742F8CE6480732345988D77667FAE3F76DB5FD057AD410AD&originRegion=eu-west-1&originCreation=20220803091338}{An empirical evaluation of the comprehensibility of decision table, tree and rule based predictive models}\\

\href{https://arxiv.org/pdf/2107.02624.pdf}{UNDERSTANDING CONSUMER PREFERENCES FOR
EXPLANATIONS GENERATED BY XAI ALGORITHMS}
\begin{itemize}
    \item psychology department who are experienced in preference students?
\item marketing department, Nathalie Dens?
\item education science / manama on education
-\item find someone who does something similar
\end{itemize}


\href{https://pages.stern.nyu.edu/~fprovost/Papers/MartensProvost_Explaining.pdf}{EXPLAINING DATA-DRIVEN DOCUMENT CLASSIFICATIONS}
Check out Figure 6 on page 21
